Accounting for missing actors in interaction network inference from abundance data

Network inference aims at unraveling the dependency structure relating jointly observed variables. Graphical models provide a general framework to distinguish between marginal and conditional dependency. Unobserved variables (missing actors) may induce apparent conditional dependencies.In the context of count data, we introduce a mixture of Poisson log-normal distributions with tree-shaped graphical models, to recover the dependency structure, including missing actors. We design a variational EM algorithm and assess its performance on synthetic data. We demonstrate the ability of our approach to recover environmental drivers on two ecological datasets. The corresponding R package is available from github.com/Rmomal/nestor.

==> commands.tex <==
% Environment
\renewcommand{\appendixname}{Annex}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{remark}{Remark}
\renewcommand{\abstractname}{Summary} 
\definecolor{red1}{RGB}{228,26,28}
\definecolor{red2}{RGB}{251,180,174}
\definecolor{blue1}{RGB}{55,126,184}
\definecolor{blue2}{RGB}{179,205,227}
\definecolor{aqua2}{RGB}{0,161,108}
\definecolor{aqua1}{RGB}{151,217,195}

 
\newcommand{\RM}[2]{\textcolor{aqua1}{\sout{#1}}\textcolor{aqua2}{#2}} % Raph
\newcommand{\SR}[2]{\textcolor{gray}{#1}\textcolor{blue}{#2}} % SR

\newcommand\independent{\protect\mathpalette{\protect\independenT}{\perp}}
\newcommand{\STAB}[1]{\begin{tabular}{@{}c@{}}#1\end{tabular}}

% Functions
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\Esp}{\mathbb{E}}
\DeclareMathOperator*{\Var}{\mathbb{V}}
\DeclareMathOperator*{\Cov}{\mathbb{C}\text{ov}}
\DeclareMathOperator*{\prob}{\mathds{P}}
\DeclareMathOperator*{\probt}{\widetilde{\mathds{P}}}

% Notations pairs
\newcommand\jk{{jk}}

% Notations cal
\newcommand\Ccal{\mathcal{C}}
\newcommand\Ncal{\mathcal{N}}
\newcommand\Pcal{\mathcal{P}}
\newcommand\Tcal{\mathcal{T}}
\newcommand\mt{\widetilde{m}}
\newcommand\St{\widetilde{S}}
\newcommand\mbt{\widetilde{\bf m}}
\newcommand\Sbt{\widetilde{\bf S}}

% Notations bf
\newcommand\gammab{{\boldsymbol{\gamma}}}
\newcommand\betab{{\boldsymbol{\beta}}}
\newcommand\thetab{{\boldsymbol{\theta}}}
\newcommand\Sigmab{{\boldsymbol{\Sigma}}}
\newcommand\cst{\text{cst}}
\newcommand\Ob{{\bf O}}
\newcommand\Hb{{\bf H}}
\newcommand\Mb{{\bf M}}
\newcommand\Qb{{\bf Q}}
\newcommand\Wb{{\bf W}}
\newcommand\Xb{{\bf X}}
\newcommand\xb{{\bf x}}
\newcommand\Yb{{\bf Y}}
\newcommand\Zb{{\bf Z}}
\newcommand\zb{{\bf z}}



% Notations tilde
\newcommand\Pt{\widetilde{P}}
\newcommand\pt{\widetilde{p}}
\newcommand\et{\widetilde{\mathds{E}}}
\newcommand\e{{\mathds{E}}}
% TikZ
\newcommand{\nodesize}{1em}
\newcommand{\edgeunit}{4*\nodesize}
\tikzstyle{covariate}=[draw, rectangle, minimum width=\nodesize, minimum height=\nodesize, inner sep=0, color=black]
\tikzstyle{covmiss}=[draw, minimum width=\nodesize, minimum height=\nodesize, inner sep=0, color=gray, text=gray]
\tikzstyle{observed}=[draw, circle, minimum width=\nodesize, inner sep=0, color=black]
\tikzstyle{edge}=[-, line width=1pt, color=black]
\tikzstyle{edgemiss}=[-, line width=1pt, dashed, color=gray]


==> discussion.tex <==
\section{Discussion}
Espérance du complément de Schur $\widehat{\Omega}_{Tm} = \widehat{\Omega}_{TOO} - \widehat{\Omega}_{TOH}\widehat{\Omega}_{TH}^{-1}\widehat{\Omega}_{THO}$:
\begin{align*}
    \widehat{\Omega}_{Tkl} &= -I_{Tkl} \frac{\rho_{kl}}{1-\rho_{kl}^2}\\
    \widehat{\Omega}_{Thh} &= 1+\sum_k I_{Tkh} \frac{\rho_{kh}^2}{1-\rho_{kh}^2}
\end{align*}
Donc:
\begin{align*}
    [\widehat{\Omega}_{TOH}\widehat{\Omega}_{TH}^{-1}\widehat{\Omega}_{THO}]_{kl} &= \sum_{h\in H} I_{Tkh} \frac{\rho_{kh}}{1-\rho_{kh}^2} I_{Thl} \frac{\rho_{hl}}{1-\rho_{hl}^2} \times \frac{1}{1+\sum_j I_{Tjh} \frac{\rho_{jh}^2}{1-\rho_{jh}^2}}
\end{align*}

\paragraph{Vraisemblance CV par Monte-Carlo (V1).}
\begin{enumerate}
\item On ajuste le modèle sur une proportion $1 - 1/V$ des données : $Y_{train_v}$
\item On obtient $\widehat{\beta}$, $\widehat{\omega}_{kl}$, , $\widehat{\theta}$
\item On fait $B = 10^3$ tirages comme suit
\begin{itemize}
\item on tire $T^b \sim p_{\widehat{\beta}}(T)$ (\textcolor{red}{comment ?})
\item on extrait $\widehat\Omega_{T^b}$ et on calcule $\widehat\Sigma_{T^bm}$ 
\item on tire $U^b_O \sim \Ncal(0, \widehat\Sigma_{T^bm})$
\item on calcule $p(Y_{test_v} | U^b_O; \widehat{\theta})$
\end{itemize}
\item on calcule le critère moyenné $Crit = V^{-1} Crit_v$ avec
\begin{align*}
Crit_v 
& = \frac1B \sum_b p(Y_{test_v} | U^b_O, T^b; \widehat{\theta}) \\
& \approx \widehat{\Esp}_{T, U_0; \widehat{\beta}, \widehat{\omega}} p(Y_{test_v} | U^b_O, T^b; \widehat{\theta}) = \widehat{p}(Y_{test_v}; \widehat{\beta}, \widehat{\omega}, \widehat{\theta})
\end{align*}
\end{enumerate}

\paragraph{Vraisemblance CV par Monte-Carlo (V2).}
On veut éviter l'intégration sur les cachées
\begin{enumerate}
\item On ajuste le modèle sur une proportion $1 - 1/V$ des données : $Y^v_{train}$
\item On obtient $\widehat{\beta}$, $\widehat{\omega}_{kl}$, , $\widehat{\theta}$
\item On fait $B$ tirages comme suit
\begin{itemize}
\item on tire $T^b \sim p_{\widehat{\beta}}(T)$
\item on extrait $\widehat\Omega_{T^b}$ et on calcule $\widehat\Sigma_{T^bm}$ 
\item pour chaque site test $i$ et chaque paire d'espèces $(j, k)$, on calcule la densité Poisson log-normale $p_{PLN}((Y_{ij}, Y_{ik}) | T^b; \widehat{\theta})$
\end{itemize}
\item on calcule le critère moyenné $Crit = V^{-1} Crit_v$ avec
\begin{align*}
Crit_v 
& = \frac1B \sum_b \sum_{i \in test_v} \sum_{j < k} \log p_{PLN}((Y_{ij}, Y_{ik}) | T^b; \widehat{\theta})
\end{align*}
\end{enumerate}


%library(tidyverse)
%library(tidymodels)


% folds<-vfold_cv(tab, v = 10) 
% performance<-map_dfr(folds$splits,
%         function(x) {
%           x.train<-as_tibble(x,data = "analysis")
%           x.test <-as_tibble(x,data = "assessment")
%           res=glm(chd~.,family=binomial,data=x.train);
%           yprob <-predict(res,newdata=x.test,type="response");
%           perf<- mean( (yprob>0.5) == x.test$chd )
%           confusion.matrix=table(yprob>0.5,x.test$chd);
%           errors<-1-diag(confusion.matrix)/colSums(confusion.matrix)
%           tibble(perf=perf,FN=errors[1],FP=errors[2])
%         })
% performance<-gather(performance,key="Criterion",value="Value")
% ggplot(data=performance,aes(x=Criterion,y=Value,col=Criterion)) + geom_boxplot()

==> model_JDS.tex <==
%\section{Model}

%\paragraph{Poisson log-normal model.} 
%We begin with a reminder on the Poisson log-normal model (PLN) model with the example of abundance data. The abundances of $p$ species sampled on $n$ sites are gathered in the matrix $n \times p$ $\Ybf$ where $Y_ {ij}$ is the abundance of species $j$ at site $i$, and $\Ybf_i $ is the abundance vector sampled on site $i$ ($i^{\text{th}}$ row of $\Ybf$). A covariate vector $\xbf_i $ of size $d$ is measured on each site $i$ and all covariates are gathered in matrix $n \times d$ $\boldsymbol X$. The PLN model states that a (latent) Gaussian vector $\Zbf_i$ of size $p$ is associated to each site:
%\begin{equation} \label{eq:PLN-Z}
%\{\Zbf_i\}_{1 \leq i \leq n} \text{ iid}, \qquad 
%\Zbf_1 \sim \Ncal_p(\zerobf, \Omegabf^{-1}),
%\end{equation}
%sites are thus assumed to be independent. All latent vectors $\Zbf_i$ are gathered in a matrix $n \times p$ written $\Zbf$. The PLN model further assumes that species abundances in all sites are conditionally independent, and their distribution depend on the environment and the associated latent variable as follows:
%\begin{equation} \label{eq:PLN-Y.Z}
%\{Y_{ij}\}_{1 \leq i \leq n, 1 \leq j \leq p} \mid \Zbf \text{ iid}, \qquad 
%Y_{ij} \mid \Zbf \sim \Pcal\left(\exp(o_{ij} + \xbf_i^\intercal \thetabf_j + Z_{ij})\right),
%\end{equation}
%where $o_{ij}$ is a known offset term which accounts for sampling effort. The vector $d \times 1$ of regression coefficients $\thetabf_j$ describes the environment effect $\xbf_i$ on species $j$. The dependence between the species abundances is entirely controlled by the latent dependency structure encoded in $\Omegabf$.

%\paragraph{Sparse dependency structure.} 
%Network inference generally relies on the hypothesis that few species are directly dependent on one another, meaning that the underlying graphical model is sparse. A way to foster such sparsity is to impose to the precision matrix $\Omegabf$ to be faithful to a spanning tree $T$ (thus $\Zbf_1 \sim \Ncal_p(\zerobf, \Omegabf_T^{-1})$ where non-nul terms of $\Omegabf_T$ correspond to $T$ edges). However this hypothesis is very restrictive  as it allows only $p-1$ links among $p$ species \citep{ChowLiu}. A more flexible approach consists in assuming that the latent vectors are drawn from a mixture of Gaussian laws, each faithful to a tree $T$:
%\begin{equation} \label{eq:mixt-Z}
%\Zbf_1 \sim \sum_{T \in \Tcal_p} \pi_T \Ncal_p(\zerobf, \Omegabf_T^{-1}),
%\end{equation}
%where $\Tcal_p$ is the space of spanning trees with $p$ nodes. Assuming furthermore that the law on trees $\{\pi_T\}_{T \in \Tcal_p}$ can be written as a product on the edges:
%\begin{equation} \label{eq:prob-T}
%\pi_T = \left. \prod_{(j, k) \in T} \beta_{jk} \right/ B, \qquad
%B = \sum_{T \in \Tcal_p} \prod_{(j, k) \in T} \beta_{jk},
%\end{equation}
%then the inference of such model is accessible from a computational point of view thanks to the Matrix tree theorem, which allows to compute a quantity of the form of ^$B$ in  $O(p^3)$ \citep{matrixtree,MeilaJaak,kirshner}. The probability of a tree is then proportional to the product of its edges weights $\{\beta_{jk}\}_{(j,k)\in T}$.

%\paragraph{Introducing missing actors.} 

%Assuming $r$ missing actors in the model, the latent vector $\Zbf_i$ associated to site $i$ is in fact of size $(p+r)$ and can be decomposed in $\Zbf_i^\intercal = [\Zbf_{Oi}^\intercal, \Zbf_{Hi}^\intercal]^\intercal$ where $\Zbf_{Oi}$ is of size $p$ and correspond to observed species and $\Zbf_{Hi}$ is of size $r$ and correspond to missing actors (species or others). The model then states that

%\begin{enumerate}[($i$)]
%\item  Abundance vectors $\Ybf_i$ of the  $p$ observed species are distributed according to \eqref{eq:PLN-Y.Z}, replacing $\Zbf$ with $\Zbf_O$,
%\item   $\Zbf_i$ is distributed according to the mixture described by\eqref{eq:mixt-Z} and \eqref{eq:prob-T} but with Gaussians of dimension $(p+r)$, and trees drawn from $\Tcal_{p+r}$.
%\end{enumerate}
%Figure \ref{MG}b) gives the graphical model associated to this model. Observed data $\Ybf$ are independent from the tree  $T$ conditionally on latent covariates $\Zbf=(\Zbf_O,\Zbf_H)$, and their conditional distribution only depends on $\Zbf_O$. Thus $\Zbf_O$ is the latent part associated to observed data while no observed data is directly linked to the   $\Zbf_H$ part.

%Finally, the original PLN model only concerns covariates $\Ybf$ and $\Zbf_O$. The use of a dependency structure with mixture of trees allows a sparse and efficient inference, and missing actors are accounted for in covariate $\Zbf_H$.
